An Ensemble of Epoch-wise Empirical Bayes for Few-shot Learning

Few-shot learning aims to train efficient predictive models with a few examples. The lack of training data leads to poor models that perform high-variance or low-confidence predictions. In this paper, we propose to meta-learn the ensemble of epoch-wise empirical Bayes models (E3BM) to achieve robust predictions. "Epoch-wise" means that each training epoch has a Bayes model whose parameters are specifically learned and deployed. "Empirical" means that the hyperparameters, e.g., used for learning and ensembling the epoch-wise models, are generated by hyperprior learners conditional on task-specific data. We introduce four kinds of hyperprior learners by considering inductive vs. transductive, and epoch-dependent vs. epoch-independent, in the paradigm of meta-learning. We conduct extensive experiments for five-class few-shot tasks on three challenging benchmarks: miniImageNet, tieredImageNet, and FC100, and achieve top performance using the epoch-dependent transductive hyperprior learner, which captures the richest information. Our ablation study shows that both "epoch-wise ensemble" and "empirical" encourage high efficiency and robustness in the model performance.

==> misc/5_mini_1shot_value_alpha_v.tex <==
\begin{figure}

\begin{center}
\subfigure[learning rate $\alpha$]{\includegraphics[height=1.1in]{misc/file_new/plot_alpha_mini_1shot.eps}}
\subfigure[combination weight $v$]{\includegraphics[height=1.1in]{misc/file_new/plot_v_mini_1shot_1.eps}}
\end{center}

\caption{The values of $\alpha$ and $v$ generated by $\Psi_{\alpha}$ and $\Psi_v$, respectively. The setting is using MTL+E$^3$BM, on \emph{mini}ImageNet $1$-shot. The plots of other settings are in the supplementary. %(Fig.\thinspace\ref{plot_all_alpha_v}).
}

\label{plot_mini_1shot_alpha_v}

\end{figure}
